A Contracting Fractal Group, Schreier Graphs and The Spectra

This paper explores a previously uncharted automaton group generated by a 5-state automaton $(\Pi, A)$ acts by self-similarity on the regular rooted tree $A^{*}$ over a 2-letter alphabet set $A$. Group $G$ has been subjected to several observations that reveal the self-similar $G$-action possesses several notable characteristics: it is a weak branch, contracting, fractal group, and satisfies the open set condition with an exponential growth rate in activity. The corresponding Schreier graphs $\Gamma$ of the group action on the binary rooted tree, for $n\leq 12$, are presented. Furthermore, we delve into a numerical approximation of the spectrum of the discrete Laplacian operator, which is defined on the limit Schreier graph $\hat{\Gamma}=\lim_{n\rightarrow\infty} \Gamma_{n}$.

==> ref.tex <==
%% Journal article
@article{barre2007real,
  title={Real and discrete holomorphy: Introduction to an algebraic approach},
  author={Barr{\'e}, Sylvain and Zeghib, Abdelghani},
  journal={Journal de math{\'e}matiques pures et appliqu{\'e}es},
  volume={87},
  number={5},
  pages={495--513},
  year={2007},
  publisher={Elsevier}
}
@article{gromov1999topological,
  title={Topological invariants of dynamical systems and spaces of holomorphic maps: I},
  author={Gromov, Misha},
  journal={Mathematical Physics, Analysis and Geometry},
  volume={2},
  number={4},
  pages={323--415},
  year={1999},
  publisher={Kluwer Academic Publishers}
}
@book{ceccherini2010cellular,
  title={Cellular automata and groups},
  author={Ceccherini-Silberstein, Tullio and Coornaert, Michel},
  volume={36},
  year={2010},
  publisher={Springer}
}
@article{nordin2020orbit,
  title={Orbit growth of Dyck and Motzkin shifts via Artin--Mazur zeta function},
  author={Nordin, Azmeer and Md Noorani, Mohd Salmi and Che Dzul-Kifli, Syahida},
  journal={Dynamical Systems},
  volume={35},
  number={4},
  pages={655--667},
  year={2020},
  publisher={Taylor \& Francis}
}
@article{kesten1959symmetric,
  title={Symmetric random walks on groups},
  author={Kesten, Harry},
  journal={Transactions of the American Mathematical Society},
  volume={92},
  number={2},
  pages={336--354},
  year={1959},
  publisher={JSTOR}
}
@article{grigorchuk1999asymptotic,
  title={On the asymptotic spectrum of random walks on infinite families of graphs},
  author={Grigorchuk, Rostislav I and Zuk, Andrzej},
  journal={Random walks and discrete potential theory (Cortona, 1997)},
  pages={188--204},
  year={1999}
}
@article{grigorchuk2012spectral,
  title={The spectral measure of the Markov operator related to 3-generated 2-group of intermediate growth and its Jacobi parameters},
  author={Grigorchuk, Rostislav Ivanovich and Krylyuk, Ya S},
  journal={Algebra and discrete mathematics},
  number={13,№ 2},
  pages={237--272},
  year={2012},
  publisher={Institute of Applied Mathematics and Mechanics of the National Academy of~…}
}
@article{grigorchuk2021spectra,
  title={Spectra of Cayley graphs of the lamplighter group and random Schr{\"o}dinger operators},
  author={Grigorchuk, Rostislav and Simanek, Brian},
  journal={Transactions of the American Mathematical Society},
  volume={374},
  number={4},
  pages={2421--2445},
  year={2021}
}
@book{nekrashevych2005self,
  title={Self-similar groups},
  author={Nekrashevych, Volodymyr},
  number={117},
  year={2005},
  publisher={American Mathematical Soc.}
}
@article{bartholdi1999spectrum,
  title={On the spectrum of Hecke type operators related to some fractal groups},
  author={Bartholdi, Laurent and Grigorchuk, Rostislav I},
  journal={arXiv preprint math/9910102},
  year={1999}
}
@article{bartholdi2000spectra,
  title={Spectra of non-commutative dynamical systems and graphs related to fractal groups},
  author={Bartholdi, Laurent and Grigorchuk, Rostislav I},
  journal={Comptes Rendus de l'Acad{\'e}mie des Sciences-Series I-Mathematics},
  volume={331},
  number={6},
  pages={429--434},
  year={2000},
  publisher={Elsevier}
}
@book{totaro2014group,
  title={Group cohomology and algebraic cycles},
  author={Totaro, Burt},
  number={204},
  year={2014},
  publisher={Cambridge University Press}
}
@book{bass2006cyclic,
  title={Cyclic renormalization and automorphism groups of rooted trees},
  author={Bass, Hyman and Otero-Espinar, Maria V and Rockmore, Daniel and Tresser, Charles},
  year={2006},
  publisher={Springer}
}
@book{ceccherini2010representation,
  title={Representation theory of the symmetric groups: the Okounkov-Vershik approach, character formulas, and partition algebras},
  author={Ceccherini-Silberstein, Tullio and Scarabotti, Fabio and Tolli, Filippo},
  volume={121},
  year={2010},
  publisher={Cambridge University Press}
}
@article{bekka2016spectral,
  title={Spectral rigidity of group actions on homogeneous spaces},
  author={Bekka, Bachir},
  journal={arXiv preprint arXiv:1602.02892},
  year={2016}
}
@book{figa1991harmonic,
  title={Harmonic analysis and representation theory for groups acting on homogenous trees},
  author={Fig{\`a}-Talamanca, Alessandro and Nebbia, Claudio},
  volume={162},
  year={1991},
  publisher={Cambridge University Press}
}
@article{ceccherini2006trees,
  title={Trees, wreath products and finite Gelfand pairs},
  author={Ceccherini-Silberstein, Tullio and Scarabotti, Fabio and Tolli, Filippo},
  journal={Advances in Mathematics},
  volume={206},
  number={2},
  pages={503--537},
  year={2006},
  publisher={Elsevier}
}
@article{d2009group,
  title={A group of automorphisms of the rooted dyadic tree and associated Gelfand pairs},
  author={D’Angeli, Daniele and Donno, Alfredo},
  journal={Rendiconti del Seminario Matematico della Universit{\`a} di Padova},
  volume={121},
  pages={73--92},
  year={2009}
}
@article{ceccherini2007finite,
  title={Finite Gel’fand pairs and their applications to probability and statistics},
  author={Ceccherini-Silberstein, T and Scarabotti, F and Tolli, F},
  journal={Journal of Mathematical Sciences},
  volume={141},
  number={2},
  pages={1182--1229},
  year={2007},
  publisher={Springer}
}
@article{d2007self,
  title={Self-similar groups and finite Gelfand pairs},
  author={D’Angeli, Daniele and Donno, Alfredo},
  journal={Algebra and Discrete Mathematics},
  year={2007},
  publisher={Інститут прикладної математики і механіки НАН України}
}
@incollection{ceccherini2009finite,
  title={Finite Gelfand pairs: examples and applications},
  author={Ceccherini-Silberstein, Tullio and D'ANGELI, DANIELE and Donno, Alfredo and Scarabotti, Fabio and Tolli, Filippo},
  booktitle={Ischia group theory 2008},
  pages={7--41},
  year={2009},
  publisher={World Scientific}
}
@incollection{bartholdi2003fractal,
  title={From fractal groups to fractal sets},
  author={Bartholdi, Laurent and Grigorchuk, Rostislav and Nekrashevych, Volodymyr},
  booktitle={Fractals in Graz 2001},
  pages={25--118},
  year={2003},
  publisher={Springer}
}
@book{ratcliffe1994foundations,
  title={Foundations of hyperbolic manifolds},
  author={Ratcliffe, John G and Axler, S and Ribet, KA},
  volume={149},
  year={1994},
  publisher={Springer}
}
@book{bridson2013metric,
  title={Metric spaces of non-positive curvature},
  author={Bridson, Martin R and Haefliger, Andr{\'e}},
  volume={319},
  year={2013},
  publisher={Springer Science \& Business Media}
}
@article{bartholdi2006automata,
  title={Automata, groups, limit spaces, and tilings},
  author={Bartholdi, Laurent and Henriques, Andr{\'e} G and Nekrashevych, Volodymyr V},
  journal={Journal of Algebra},
  volume={305},
  number={2},
  pages={629--663},
  year={2006},
  publisher={Elsevier}
}
@book{kigami2001analysis,
  title={Analysis on fractals},
  author={Kigami, Jun},
  number={143},
  year={2001},
  publisher={Cambridge University Press}
}
@article{grigorchuk2011some,
  title={Some topics in the dynamics of group actions on rooted trees},
  author={Grigorchuk, Rostislav I},
  journal={Proceedings of the Steklov Institute of Mathematics},
  volume={273},
  number={1},
  pages={64--175},
  year={2011},
  publisher={Springer}
}
@article{bartholdi1999parabolic,
  title={On parabolic subgroups and Hecke algebras of some fractal groups},
  author={Bartholdi, Laurent and Grigorchuk, Rostislav I},
  journal={arXiv preprint math/9911206},
  year={1999}
}
@article{grigorchuk2018spectra,
  title={Spectra of Schreier graphs of Grigorchuk’s group and Schroedinger operators with aperiodic order},
  author={Grigorchuk, Rostislav and Lenz, Daniel and Nagnibeda, Tatiana},
  journal={Mathematische Annalen},
  volume={370},
  number={3},
  pages={1607--1637},
  year={2018},
  publisher={Springer}
}
@article{grigorchuk2001lamplighter,
  title={The lamplighter group as a group generated by a 2-state automaton, and its spectrum},
  author={Grigorchuk, Rostislav I and {\.Z}uk, Andrzej},
  journal={Geometriae Dedicata},
  volume={87},
  number={1},
  pages={209--244},
  year={2001},
  publisher={Springer}
}
@article{nekrashevych2008groups,
  title={Groups and analysis on fractals},
  author={Nekrashevych, Volodymyr and Teplyaev, Alexander},
  journal={Analysis on graphs and its applications},
  volume={77},
  pages={143--180},
  year={2008},
  publisher={Citeseer}
}
@article{donno2013constructing,
  title={Constructing Laplacians on Limit Spaces of Self-similar Groups},
  author={Donno, Alfredo},
  journal={Trends in Harmonic Analysis},
  pages={245--275},
  year={2013},
  publisher={Springer}
}
@article{grigorchuk2004ihara,
  title={The Ihara zeta function of infinite graphs, the KNS spectral measure and integrable maps},
  author={Grigorchuk, Rostislav I and Zuk, Andrzej},
  journal={Random walks and geometry},
  pages={141--180},
  year={2004},
  publisher={Walter de Gruyter GmbH \& Co. KG Berlin}
}
@article{bondarenko2008classification,
  title={Classification of groups generated by 3-state automata over a 2-letter alphabet},
  author={Bondarenko, Ievgen and Grigorchuk, Rostislav and Kravchenko, Rostyslav and Muntyan, Yevgen and Nekrashevych, Volodymyr and Savchuk, Dmytro and Sunic, Zoran},
  journal={arXiv preprint arXiv:0803.3555},
  year={2008}
}
@incollection{gromov1987hyperbolic,
  title={Hyperbolic groups},
  author={Gromov, Mikhael},
  booktitle={Essays in group theory},
  pages={75--263},
  year={1987},
  publisher={Springer}
}
@article{kapovich2002boundaries,
  title={Boundaries of hyperbolic groups},
  author={Kapovich, Ilya and Benakli, Nadia},
  journal={arXiv preprint math/0202286},
  year={2002}
}
@article{bondarenko2008classification,
  title={Classification of groups generated by 3-state automata over a 2-letter alphabet},
  author={Bondarenko, Ievgen and Grigorchuk, Rostislav and Kravchenko, Rostyslav and Muntyan, Yevgen and Nekrashevych, Volodymyr and Savchuk, Dmytro and Sunic, Zoran},
  journal={arXiv preprint arXiv:0803.3555},
  year={2008}
}
@article{delyon1991recurrence,
  title={Recurrence of the eigenstates of a Schr{\"o}dinger operator with automatic potential},
  author={Delyon, F and Peyriere, J},
  journal={Journal of statistical physics},
  volume={64},
  number={1},
  pages={363--368},
  year={1991},
  publisher={Springer}
}
@incollection{bellissard1992gap,
  title={Gap labelling theorems for Schr{\"o}dinger operators},
  author={Bellissard, Jean},
  booktitle={From number theory to physics},
  pages={538--630},
  year={1992},
  publisher={Springer}
}
@article{avron1981almost,
  title={Almost periodic Schroedinger operators. Pt. 1},
  author={Avron, J and Simon, B},
  journal={Communications in Mathematical Physics},
  volume={82},
  number={1},
  pages={101--120},
  year={1981}
}
@article{simon2008schrodinger,
  title={Schrodinger Operators with Purely Discrete Spectrum},
  author={Simon, Barry},
  journal={arXiv preprint arXiv:0810.3275},
  year={2008}
}
@article{sy1992discrete,
  title={Discrete Schr{\"o}dinger operators on a graph},
  author={Sy, Polly Wee and Sunada, Toshikazu},
  journal={Nagoya Mathematical Journal},
  volume={125},
  pages={141--150},
  year={1992},
  publisher={Cambridge University Press}
}
@incollection{sunada1988fundamental,
  title={Fundamental groups and Laplacians},
  author={Sunada, Toshikazu},
  booktitle={Geometry and analysis on manifolds},
  pages={248--277},
  year={1988},
  publisher={Springer}
}
@article{grigorchuk2018spectra,
  title={Spectra of Schreier graphs of Grigorchuk’s group and Schroedinger operators with aperiodic order},
  author={Grigorchuk, Rostislav and Lenz, Daniel and Nagnibeda, Tatiana},
  journal={Mathematische Annalen},
  volume={370},
  number={3},
  pages={1607--1637},
  year={2018},
  publisher={Springer}
}
@article{grigorchuk2017schreier,
  title={Schreier graphs of Grigorchuk’s group and a subshift associated to a nonprimitive substitution},
  author={Grigorchuk, Rostislav and Lenz, Daniel and Nagnibeda, Tatiana},
  journal={Groups, graphs and random walks},
  volume={436},
  pages={250--299},
  year={2017},
  publisher={Cambridge University Press Cambridge}
}
@article{bondarenko2007post,
  title={Post-critically finite self-similar groups},
  author={Bondarenko, Ievgen and Nekrashevych, Volodymyr},
  journal={arXiv preprint math/0701824},
  year={2007}
}
@article{grigorchuk2020spectra,
  title={On spectra and spectral measures of Schreier and Cayley graphs},
  author={Grigorchuk, Rostislav and Nagnibeda, Tatiana and P{\'e}rez, Aitor},
  journal={arXiv preprint arXiv:2007.03309},
  year={2020}
}
@article{ju2012post,
  title={Post-critically finite fractal and Martin boundary},
  author={Ju, Hongbing and Lau, Ka-Sing and Wang, Xiang-Yang},
  journal={Transactions of the American Mathematical Society},
  volume={364},
  number={1},
  pages={103--118},
  year={2012}
}
@article{bondarenko2011ends,
  title={Ends of Schreier graphs of self-similar groups},
  author={Bondarenko, Ievgen and D’Angeli, Daniele and Nagnibeda, Tatiana},
  journal={preprint},
  year={2011}
}
@article{bondarenko2011graph,
  title={Graph-directed systems and self-similar measures on limit spaces of self-similar groups},
  author={Bondarenko, Ievgen V and Kravchenko, Rostyslav V},
  journal={Advances in Mathematics},
  volume={226},
  number={3},
  pages={2169--2191},
  year={2011},
  publisher={Elsevier}
}
@incollection{bass2001tree,
  title={Tree lattices},
  author={Bass, Hyman and Lubotzky, Alexander},
  booktitle={Tree Lattices},
  pages={25--33},
  year={2001},
  publisher={Springer}
}
@article{bass1992ihara,
  title={The Ihara-Selberg zeta function of a tree lattice},
  author={Bass, Hyman},
  journal={International Journal of Mathematics},
  volume={3},
  number={06},
  pages={717--797},
  year={1992},
  publisher={World Scientific}
}
@article{bass1993covering,
  title={Covering theory for graphs of groups},
  author={Bass, Hyman},
  journal={Journal of pure and applied algebra},
  volume={89},
  number={1-2},
  pages={3--47},
  year={1993},
  publisher={Elsevier}
}
@incollection{serre1979local,
  title={Local class field theory},
  author={Serre, Jean-Pierre},
  booktitle={Local Fields},
  pages={188--203},
  year={1979},
  publisher={Springer}
}
@book{serre2002trees,
  title={Trees},
  author={Serre, Jean-Pierre},
  year={2002},
  publisher={Springer Science \& Business Media}
}
@techreport{gromov1992asymptotic,
  title={Asymptotic invariants of infinite groups},
  author={Gromov, Mikhael},
  year={1992},
  institution={P00001028}
}
@article{gromov1981groups,
  title={Groups of polynomial growth and expanding maps (with an appendix by Jacques Tits)},
  author={Gromov, Michael},
  journal={Publications Math{\'e}matiques de l'IH{\'E}S},
  volume={53},
  pages={53--78},
  year={1981}
}
@inproceedings{gromov1980hyperbolic,
  title={Hyperbolic manifolds, groups and actions},
  author={Gromov, Mikhael},
  booktitle={Riemann surfaces and related topics: Proceedings of the 1978 Stony Brook Conference (State Univ. New York, Stony Brook, NY, 1978)},
  volume={97},
  pages={183--213},
  year={1980}
}
@article{simon2001hausdorff,
  title={Hausdorff dimension of limit sets for parabolic IFS with overlaps},
  author={Simon, K{\'a}roly and Solomyak, Boris and Urba{\'n}ski, M},
  journal={Pacific journal of mathematics},
  volume={201},
  number={2},
  pages={441--478},
  year={2001},
  publisher={Mathematical Sciences Publishers}
}
@article{gel1952geodesic,
  title={Geodesic flows on manifolds of constant negative curvature},
  author={Gel'fand, Izrail Moiseevich and Fomin, Sergei Vasil'evich},
  journal={Uspekhi Matematicheskikh Nauk},
  volume={7},
  number={1},
  pages={118--137},
  year={1952},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian~…}
}
@incollection{anosov2020ergodic,
  title={Ergodic properties of geodesic flows on closed Riemannian manifolds of negative curvature},
  author={Anosov, Dmitry Victorovich},
  booktitle={Hamiltonian Dynamical Systems},
  pages={486--489},
  year={2020},
  publisher={CRC Press}
}
@article{anosov1967geodesic,
  title={Geodesic flows on closed Riemannian manifolds of negative curvature},
  author={Anosov, Dmitry Victorovich},
  journal={Trudy Matematicheskogo Instituta Imeni VA Steklova},
  volume={90},
  pages={3--210},
  year={1967},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian~…}
}
@article{hopf1971ergodic,
  title={Ergodic theory and the geodesic flow on surfaces of constant negative curvature},
  author={Hopf, Eberhard},
  journal={Bulletin of the American Mathematical Society},
  volume={77},
  number={6},
  pages={863--877},
  year={1971},
  publisher={American Mathematical Society}
}
@article{yue1996ergodic,
  title={The ergodic theory of discrete isometry groups on manifolds of variable negative curvature},
  author={Yue, Chengbo},
  journal={Transactions of the American Mathematical Society},
  volume={348},
  number={12},
  pages={4965--5005},
  year={1996}
}
@article{jezouin2013quantum,
  title={Quantum limit of heat flow across a single electronic channel},
  author={Jezouin, S{\'e}bastien and Parmentier, FD and Anthore, A and Gennser, U and Cavanna, A and Jin, Yong and Pierre, F},
  journal={Science},
  volume={342},
  number={6158},
  pages={601--604},
  year={2013},
  publisher={American Association for the Advancement of Science}
}
@article{bourgain2003entropy,
  title={Entropy of quantum limits},
  author={Bourgain, Jean and Lindenstrauss, Elon},
  journal={Communications in mathematical physics},
  volume={233},
  number={1},
  pages={153--171},
  year={2003},
  publisher={Springer}
}
@article{anantharaman2007entropy,
  title={Entropy and localization of eigenfunctions},
  author={Anantharaman, Nalini},
  journal={S{\'e}minaire {\'E}quations aux d{\'e}riv{\'e}es partielles (Polytechnique) dit aussi" S{\'e}minaire Goulaouic-Schwartz"},
  pages={1--17},
  year={2007}
}
@article{bishop1997hausdorff,
  title={Hausdorff dimension and Kleinian groups},
  author={Bishop, Christopher J and Jones, Peter W},
  journal={Acta Mathematica},
  volume={179},
  number={1},
  pages={1--39},
  year={1997},
  publisher={Institut Mittag-Leffler}
}
@article{d2009schreier,
  title={Schreier graphs of the Basilica group},
  author={D'angeli, Daniele and Donno, Alfredo and Matter, Michel and Nagnibeda, Tatiana},
  journal={arXiv preprint arXiv:0911.2915},
  year={2009}
}
@incollection{d2011partition,
  title={Partition functions of the Ising model on some self-similar Schreier graphs},
  author={D’Angeli, Daniele and Donno, Alfredo and Nagnibeda, Tatiana},
  booktitle={Random walks, boundaries and spectra},
  pages={277--304},
  year={2011},
  publisher={Springer}
}
@article{aleshin1972finite,
  title={Finite automata and Burnside's problem for periodic groups},
  author={Aleshin, Stanislav V},
  journal={Mathematical Notes of the Academy of Sciences of the USSR},
  volume={11},
  number={3},
  pages={199--203},
  year={1972},
  publisher={Springer}
}
@book{margulis1991discrete,
  title={Discrete subgroups of semisimple Lie groups},
  author={Margulis, Gregori A},
  volume={17},
  year={1991},
  publisher={Springer Science \& Business Media}
}
@article{lenz2002uniform,
  title={Uniform ergodic theorems on subshifts over a finite alphabet},
  author={Lenz, Daniel},
  journal={Ergodic Theory and Dynamical Systems},
  volume={22},
  number={1},
  pages={245--255},
  year={2002},
  publisher={Cambridge University Press}
}
@article{lavrenyuk2008lattice,
  title={Lattice of normal subgroups of a group of local isometries of the boundary of a spherically homogeneous tree.},
  author={Lavrenyuk, Ya V and Sushchanskii, VI},
  journal={Ukrainian Mathematical Journal},
  volume={60},
  number={10},
  year={2008}
}
@book{lindstrom1990brownian,
  title={Brownian motion on nested fractals},
  author={Lindstrom, Tom and Lindstr{\o}m, Tom},
  number={420},
  year={1990},
  publisher={American Mathematical Soc.}
}
@article{bowditch1998topological,
  title={A topological characterisation of hyperbolic groups},
  author={Bowditch, Brian},
  journal={Journal of the American Mathematical Society},
  volume={11},
  number={3},
  pages={643--667},
  year={1998}
}
@article{-1994,
doi	= {10.1515/crll.1994.455.57},
title	= {Ergodicity of harmonic invariant measures for the geodesic flow on hyperbolic spaces.},
journal	= {Journal für die reine und angewandte Mathematik (Crelles Journal)    1994-oct 01 vol. 1994 iss. 455},

year	= {1994},
month	= {oct},
day	= {01},
volume	= {1994},
issue	= {455},
page	= {57--104},
url =       {libgen.li/file.php?md5=50f6bc9a48d265b20890a72bf2c420af},
}
